UniverSat: Resolution- and Modality-Agnostic Transformers for Earth Observation

Vision Transformers (ViT) dominate computer vision. However, their reliance on rigid patch projectors hinders transfer to Earth Observation (EO), where input modalities, scales, and resolutions vary widely. We introduce UniverSat, a ViT-style backbone built around a Universal Patch Encoder that maps patches from arbitrary spatial, spectral, and temporal resolutions, and from both optical and non-optical sensors, into a shared embedding space with a shared set of weights. This enables training a single model on heterogeneous multimodal corpora via self-supervision, yielding robust, sensor-agnostic spatial features. We validate this approach with strong results across classification and segmentation on standard EO benchmarks from GeoBench, PANGEABench, and SpectralEarth. Our code and models are available at https://github.com/gastruc/UniverSat.

==> figures/acube.tex <==


    % Cube dimenasions
    % Grid steps
    \def\xstep{\xmax/\xdiv}
    \def\ystep{\ymax/\ydiv}
    \def\zstep{\zmax/\zdiv}

    %\node[draw=\tempdrawcolor] (0,0) {\randomcolor};
  % === Fill bottom face (z=\zmax) cell-by-cell ===
    \foreach \i in {0,...,\numexpr\xdiv-1\relax} {
        \foreach \j in {0,...,\numexpr\ydiv-1\relax} {
            % random percentage between 20 and 80
            \pgfmathsetmacro{\ip}{\i+1}
            \pgfmathsetmacro{\jp}{\j+1}
            \pgfmathsetmacro{\km}{\zdiv-1}
            \randomcellcolor{\i}{\j}{\km}
            \fill[fill=\getrandomcolor] 
                (\i*\xstep, \j*\ystep, \zmax) --
                 (\ip*\xstep, \j*\ystep, \zmax) --
                 (\ip*\xstep, \jp*\ystep, \zmax) --
                (\i*\xstep, \jp*\ystep, \zmax) -- cycle;
        }
    }

    % === Fill left face (x=\xmax) cell-by-cell ===
    \foreach \j in {0,...,\numexpr\ydiv-1\relax} {
        \foreach \k in {0,...,\numexpr\zdiv-1\relax} {
            \pgfmathsetmacro{\im}{\xdiv-1}
            \pgfmathsetmacro{\jp}{\j+1}
            \pgfmathsetmacro{\kp}{\k+1}
            \randomcellcolor{\im}{\j}{\k}
            \fill[fill=\getrandomcolor] 
                (\xmax, \j*\ystep, \k*\zstep) --
                (\xmax, \jp*\ystep, \k*\zstep) --
                (\xmax, \jp*\ystep, \kp*\zstep) --
                (\xmax, \j*\ystep, \kp*\zstep) -- cycle;
        }
    }

    % === Fill front face (y=0) cell-by-cell ===
    \foreach \i in {0,...,\numexpr\xdiv-1\relax} {
        \foreach \k in {0,...,\numexpr\zdiv-1\relax} {
        \pgfmathsetmacro{\ip}{\i+1}
        \pgfmathsetmacro{\kp}{\k+1}
            \pgfmathrandominteger{\randval}{20}{80}
            \randomcellcolor{\i}{0}{\k}

            \fill[fill=\getrandomcolor] 
                (\i*\xstep, 0, \k*\zstep) --
                (\ip*\xstep, 0, \k*\zstep) --
                (\ip*\xstep, 0, \kp*\zstep) --
                (\i*\xstep, 0, \kp*\zstep) -- cycle;
        }
    }

% === Edges ===
     \foreach \i in {1,...,\xdiv} {
        \draw[thin, draw=\color!\edgeintensity] (\i*\xstep,0,0) -- (\i*\xstep,0,\zmax);
        \draw[thin, draw=\color!\edgeintensity] (\i*\xstep,0,\zmax) -- (\i*\xstep,\ymax,\zmax);
    }
    
    \foreach \i in {1,...,\zdiv} {
        \draw[thin, draw=\color!\edgeintensity] (0,0,\i*\zstep) -- (\xmax,0,\i*\zstep);
        \draw[thin, draw=\color!\edgeintensity] (\xmax,0,\i*\zstep) -- (\xmax,\ymax,\i*\zstep);
    }
        \foreach \i in {1,...,\ydiv} {
        \draw[thin, draw=\color!\edgeintensity] (\xmax,\i*\ystep,0) -- (\xmax,\i*\ystep,\zmax);
        \draw[thin, draw=\color!\edgeintensity] (0,\i*\ystep,\zmax) -- (\xmax,\i*\ystep,\zmax);
    }
     % === Draw the three visible filled faces ===
    \draw[draw=\color, very thick] (0,0,\zmax) -- (\xmax,0,\zmax) -- (\xmax,\ymax,\zmax) -- (0,\ymax,\zmax) -- (0,0,\zmax) -- (0,0,0) -- (\xmax,0,0) -- (\xmax,\ymax,0)
    (\xmax,0,0) -- (\xmax,0,\zmax);
    \draw[draw=\color, very thick]  (\xmax,0,0) -- (\xmax,\ymax,0) -- (1.0125*\xmax,1.0125*\ymax,1.01*\zmax) ;
    
    %(\xmax,0,\zmax) -- (\xmax,\ymax,\zmax) -- (\xmax,\ymax,0) --  (\xmax,0,0) 
    % --   % Bottom face
     %\draw[draw=red, very thick]
     %(\xmax,0,0) -- (\xmax,\ymax,0) -- (\xmax,\ymax,\con*\zmax) -- (\xmax,0,\zmax) -- (\xmax,0,0);% --  % Left face
     %\draw[draw=green, very thick]
     %(0,0,0) -- (\xmax,0,0) -- (\xmax,0,\zmax) -- (0,0,\con*\zmax) -- (0,0,0) -- (\xmax/2,0,0);  % Front face

\ifnum\bigstep=2
    \foreach \i in {0,\bigstep,...,\xdiv} {
        \draw[very thick, draw=\color] (\i*\xstep,0,0) -- (\i*\xstep,0,\zmax);
        \draw[very thick, draw=\color] (\i*\xstep,0,\zmax) -- (\i*\xstep,\ymax,\zmax);
    }
    \fi

\ifnum\bigstep=4
 \ifnum\xdiv>3
    \foreach \i in {0,\bigstep,...,\xdiv} {
        \draw[very thick, draw=\color] (\i*\xstep,0,0) -- (\i*\xstep,0,\zmax);
        \draw[very thick, draw=\color] (\i*\xstep,0,\zmax) -- (\i*\xstep,\ymax,\zmax);
    }
    \fi
\fi


